A Probabilistic Framework for Modular Continual Learning

Modular approaches that use a different composition of modules for each problem are a promising direction in continual learning (CL). However, searching through the large, discrete space of module compositions is challenging, especially because evaluating a composition's performance requires a round of neural network training. We address this challenge through a modular CL framework, PICLE, that uses a probabilistic model to cheaply compute the fitness of each composition, allowing PICLE to achieve both perceptual, few-shot and latent transfer. The model combines prior knowledge about good module compositions with dataset-specific information. We evaluate PICLE using two benchmark suites designed to assess different desiderata of CL techniques. Comparing to a wide range of approaches, we show that PICLE is the first modular CL algorithm to achieve perceptual, few-shot and latent transfer while scaling well to large search spaces, outperforming previous state-of-the-art modular CL approaches on long problem sequences.

==> algorithms/v0_algorithm_pt_strategy.tex <==

\begin{algorithm}[tb] \label{alg:pt_strategy}
\SetCommentSty{\tt\small}
\DontPrintSemicolon
\SetAlgoLined
\changed{
$\mathit{paths} \gets [\,]$; $\pi \gets [\,]$\;
\For{$i \gets 1$ \KwTo $L$}{
  $\pi_{\new} \gets (m^{i+1}_{\new}, ..., m^L_{\new})$\;
  $m_i \gets \argmax_{m \in \mathcal{L}_i} p(\pi \oplus [m] \oplus \pi_{\new} \,|\, \Xtr)$\;
  Append $m_i$ to $\pi$.\;
  Append $\pi \oplus \pi_{\new}$ to $\mathit{paths}$.\;
  }
\KwRet{{paths}}\;
}
% \tcc{Sort all $M_1$ modules using KL divergence}
 \caption{Searching through perceptual-transfer paths}
\end{algorithm}




\begin{algorithm}[tb] \label{alg:npt_strategy}
\SetCommentSty{\tt\small}
\DontPrintSemicolon
\SetAlgoLined
\KwIn{A list of paths $\Pi$ that have been trained on previous tasks.}
\KwIn{A list $Y$ of the validation accuracy of each path in $\Pi$.}
\KwIn{A feature function $f(\pi, \X)$ that takes a path $\pi$ and a set of inputs $\X$ and returns a vector representation of $\pi$.}
\KwIn{The training data $(\Xtr, \Ytr)$ and validation data $(\Xval, \Yval)$ for the new task.}
\changed{
$\mathit{paths} \gets [\,]$; $\pi \gets [\,]$\;
\For{$\ell \gets \ell_{\min}$ \KwTo $L$}{
  \tcp{All suffixes of length $\ell$ from paths in $\Pi$.}
  $\Pi_\ell = \{ [m_{\ell:L}]  \text{ for each path } [m_{1:L}] \in \Pi\}$.\;  
  $\yPrev \gets [\,], \zPrev \gets [\,], \X \gets [\,]$\;
  \For{$t \gets 1$ \KwTo $T$}{ 
    \tcp{Find  best path based on the current approximate validation \st{hello} loss $p_{\text{GP}}$.}
    $\pi'_{\ell} \gets \argmax_{\pi \in \Pi_\ell} \text{UCB}(\pi, 
    p_{\text{GP}}(y \,|\, z = f(\pi, \X), \yPrev, \zPrev))$\;
    $\pi' \gets [m^{1}_{\new}, ..., m^{\ell-1}_{\new}] \oplus \pi'_{\ell}$\;\;
    $\pi^* \gets \textsc{Train}(\pi', \Xtr, \Ytr)$\;\;
    \tcp{Update the GP training set.}
    $loss \gets \textsc{ValidationLoss}(\pi^*, \Xval, \Yval)$\;
    Randomly sample $K << N$ data points from \Xtr, add to \X. \;
    Append $f(\pi^*, \X)$ to $\zPrev,$ append $\mathit{loss}$ to $\yPrev.$\;
    Append $\pi^*$ to $\mathit{paths}$.\;
  }
}
\KwRet{{paths}}\;
}
% \tcc{Sort all $M_1$ modules using KL divergence}
 \caption{Searching through nonperceptual-transfer paths}
\end{algorithm}


==> algorithms/v1_algorithm_pt_strategy.tex <==

\begin{algorithm}[tb] \label{alg:npt_strategy}
\SetCommentSty{\tt\small}
\DontPrintSemicolon
\SetAlgoLined
\KwIn{A list of paths $\Pi$ that have been trained on previous tasks.}
\KwIn{A set of inputs $\mathbf{Z}$ to the $\ell_{\min}$-th module, assembled from subsets of the training datasets of previous problems and computed using each problem's corresponding solution. \mathbf{Z} is fixed during this search.}
\KwIn{The training data $(\Xtr, \Ytr)$ and validation data $(\Xval, \Yval)$ for the new task.}
$\mathit{paths} \gets [\,]$; $\pi \gets [\,]$; \\
\changed{\tcp{Note: we only do Bayesian Optimisation for $\ell=\ell_{\min}$}}
\For{$\ell \gets \ell_{\min}$ \KwTo \changed{$\ell_{\min}$}}{
  \tcp{All suffixes of length $\ell$ from paths in $\Pi$.}
  $\Pi_\ell = \{ [m_{\ell:L}]  \text{ for each path } [m_{1:L}] \in \Pi\}$.\;  
  % $\yPrev \gets [\,], \zPrev \gets [\,], \X \gets [\,]$\;
  \changed{
  $\Gamma \gets [\,]$; $\mathbf{f} \gets [\,]$; \tcp{$\Gamma$ is evaluated NT paths, $\mathbf{f}$ is their validation performance after training.}}
  \For{$t \gets 1$ \KwTo $T$}{ 
    \tcp{Find  best \changed{\bold{unevaluated}} path based on the current approximate validation \changed{\st{loss} performance} $p_{\text{GP}}$.}
    \changed{
    $\pi'_{\ell} \gets \argmax_{\pi \in \Pi_\ell} \text{UCB}(p_{\text{GP}}(f_* | \pi, \mathbf{\Gamma}, \mathbf{f}))$ \;
    $\pi' \gets [m^{1}_{\new}, ..., m^{\ell-1}_{\new}] \oplus \pi'_{\ell}$\;
    \tcp{Technically, this algorithm only suggests the next path, and the path is trained in the Modular CL algorithm calling this sub-routine. But in effect, this is what happens.}
    }
    $\pi^* \gets \textsc{Train}(\pi', \Xtr, \Ytr)$\;\;
    \tcp{Update the GP training set.}
    \changed{
    \tcp{In the implementation we use logs.}
    $f_* = p(\Yval | \Xval ; \pi^*)$ \;
    Append $f_*$ to $\mathbf{f}$ \;
    Append $\pi'_{\ell}$ to $\Gamma$ \;
    Append $\pi'$ to $\mathit{paths}$.\;
    }
  }
}
\changed{
\tcp{Find best NT path evaluated so far.}
$i \gets \argmax_{i \in \{1, ..., T\}} \mathbf{f}[i]$ \;
$\gamma \gets \Gamma[i]$\;
Let $\lambda \in \Pi$ be original solution which $\gamma$  is the suffix of \;
\tcp{Add longer suffixes from this solution:}
\For{$\ell \gets \ell_{\min}+1$ \KwTo \changed{$L-1$}}{
    $\pi'_{\ell} \gets [m_{\ell:L}]$ from the path $\lambda$ \;
    $\pi' \gets [m^{1}_{\new}, ..., m^{\ell-1}_{\new}] \oplus \pi'_{\ell}$\;
    Append $\pi'$ to $\mathit{paths}$.\;
}
}
\KwRet{{paths}}\;

% \tcc{Sort all $M_1$ modules using KL divergence}
 \caption{Augmented: Searching through nonperceptual-transfer paths}
\end{algorithm}

